Guardians of Generation: Dynamic Inference-Time Copyright Shielding with Adaptive Guidance for AI Image Generation

Modern text-to-image generative models can inadvertently reproduce copyrighted content memorized in their training data, raising serious concerns about potential copyright infringement. We introduce Guardians of Generation, a model agnostic inference time framework for dynamic copyright shielding in AI image generation. Our approach requires no retraining or modification of the generative model weights, instead integrating seamlessly with existing diffusion pipelines. It augments the generation process with an adaptive guidance mechanism comprising three components: a detection module, a prompt rewriting module, and a guidance adjustment module. The detection module monitors user prompts and intermediate generation steps to identify features indicative of copyrighted content before they manifest in the final output. If such content is detected, the prompt rewriting mechanism dynamically transforms the user's prompt by sanitizing or replacing references that could trigger copyrighted material while preserving the prompt's intended semantics. The adaptive guidance module adaptively steers the diffusion process away from flagged content by modulating the model's sampling trajectory. Together, these components form a robust shield that enables a tunable balance between preserving creative fidelity and ensuring copyright compliance. We validate our method on a variety of generative models such as Stable Diffusion, SDXL, and Flux, demonstrating substantial reductions in copyrighted content generation with negligible impact on output fidelity or alignment with user intent. This work provides a practical, plug-and-play safeguard for generative image models, enabling more responsible deployment under real-world copyright constraints. Source code is available at: https://respailab.github.io/gog

==> sec/3_preliminaries.tex <==



 % Add this package to support theorem-like environments

% Define custom environments
\newtheorem{property}{Property}
\newtheorem{definition}{Definition}


\section{Preliminaries}
\label{sec:preliminaries}
\paragraph{Iterative Denoising Process}
During inference, the denoising process starts from a pure Guassian noise sample $x_t \sim  \mathcal{N} (0, \textbf{I})$. The model iteratively denoises this sample, conditioned on the text embedding $\textbf{e}$, to generate final output $x_0$. At inference, the denoising process iterates from \textbf{\textit{T}} to 0, . For each timestep \textit{t}, the update rule for $x_{t-1}$ is given by 

\begin{equation}
    x_{t-1}
    \;=\;
    g\bigl(
        x_{t},\, f_{\theta}(x_t,e,t),\, \beta_{t}
    \bigr),
    \label{eq:diffusion_update}
\end{equation}
where $g$ is a function that computes next latent $x_{t-1}$ given by the scheduler's update rule, $f_\theta(x_t,e,t)$ is the predicted noise at time step $t$, conditioned on text embeddings $\textbf{e}$. $\beta_t$ represents all scheduler step-dependent hyperparameters.

% In this section, we provide the necessary background on diffusion-based generative models, classifier-free guidance (CFG), and the core notations used in our work. This concise overview sets the stage for our methodology (Sec.~\ref{sec:methodology}) by clarifying the conventions, symbols, and assumptions that inform our approach.

% \paragraph{Latent Diffusion Models.}
% Let $x_t \in \mathcal{X}$ represent a latent variable at diffusion timestep $t$. In latent diffusion \cite{rombach2022high}, one typically starts with a randomly sampled latent $x_T$ (for a large $T$) and iteratively refines it toward a clean image representation $x_0$. A learned denoising function $f_{\theta}(x_t, t)$ predicts the noise present in $x_t$, and each update step (e.g., DDIM, Euler–Ancestral) computes
% \begin{equation}
%     x_{t-1}
%     \;=\;
%     g\bigl(
%         x_{t},\, f_{\theta}(x_t, t),\, \beta_{t}
%     \bigr),
%     \label{eq:diffusion_update}
% \end{equation}
% where $\beta_{t}$ indicates step-dependent hyperparameters and $g(\cdot)$ is the scheduler’s update rule. In practice, $x_0$ can be mapped to the actual image domain via a decoder or Variational Autoencoder (VAE).

\paragraph{Classifier-Free Guidance (CFG)}
Classifier-free guidance steers the generation process using textual inputs. At each timestep $t$, the denoising model generates two noise estimates: $\epsilon_{uncond}$, which is independent of the text input, and $\epsilon_{cond}$ conditioned on input $e$. The final guided prediction is calculated by interpolating between these two noise estimates, controlled by guidance scale $\eta$:

\begin{equation}
\epsilon=\epsilon_{uncond} + \eta (\epsilon_{cond} - \epsilon_{uncond})
\end{equation}
By tuning $\eta$, CFG effectively regulates the trade-off between adherence to the condition and sample diversity.

% \paragraph{Classifier-Free Guidance (CFG).}
% Classifier-free guidance \cite{ho2022classifier} is employed to steer the generation process using textual inputs. We encode a conditioning prompt $x$ into a text embedding $\phi(x)$ and generate both an \emph{unconditional} noise estimate $\epsilon_{\mathrm{uncond}}$ and a \emph{conditioned} one $\epsilon_{\mathrm{cond}}$. The final noise prediction is typically
% \begin{equation}
%     \widehat{\epsilon}
%     \;=\;
%     \epsilon_{\mathrm{uncond}}
%     \;+\;
%     \eta \,\bigl(\epsilon_{\mathrm{cond}}
%                 \;-\;
%                 \epsilon_{\mathrm{uncond}}\bigr),
%     \label{eq:cfg_update}
% \end{equation}
% where $\eta$ is a guidance scale that regulates the trade-off between faithfulness to the textual prompt and sampling diversity.

% \paragraph{Notation for Protected Concepts.}
% We maintain a finite set of protected concepts,
% \(
%     \mathcal{C}
%     \;=\;
%     \{\textit{concept}_{1}, \ldots, \textit{concept}_{m}\}.
% \)
% Each concept entry may include additional synonyms to capture semantically or lexically similar terms. We write $\mathbf{e}(x)$ to denote the embedding of a prompt $x$. A threshold $\gamma \in [0,1]$ determines when the similarity $\mathrm{sim}\bigl(\mathbf{e}(x), \mathbf{e}(\textit{concept}_{i})\bigr)$ is large enough to label $x$ as referencing $\textit{concept}_{i}$ (see also Eq.~\ref{eq:cosine} in our Methodology).

% \paragraph{LLM for Prompt Rewriting.}
% When a prompt $x$ is flagged as referencing one or more protected concepts, we invoke a large language model $\text{LLMRewrite}(\cdot)$ that removes or generalizes the flagged content while preserving relevant context. In principle, we treat the rewriting operation as a function that receives $(x, \mathcal{F}(x))$---the original prompt and the validated set of flagged concepts---and returns $x^{\prime}$. This rewriting engine is assumed to be a black box in the subsequent sections (Sec.~\ref{subsec:prompt-rewriting}), with the internal details determined by a given LLM’s capabilities.

% \paragraph{Overview of Multiple Text Encoders.}
% Although the above formulation holds generally, certain diffusion models (e.g., Stable Diffusion XL, Flux) use multiple encoders that process textual inputs differently. For instance, one encoder might be CLIP-based, while another is T5-based. Throughout our methodology, we refer to $\phi(x)$ in an abstract manner, acknowledging that, in practice, each encoder produces an embedding that is later combined or concatenated (Sec.~\ref{subsec:cfg-adaptation}).

% \smallskip
% \noindent
% \textbf{Remark.} The subsequent sections will build on these definitions to detail our pipeline’s three main stages: (i) detection of protected concepts, (ii) prompt rewriting, and (iii) adaptive CFG-based image generation. If any aspect of the above notations or assumptions requires further specialization, it is addressed contextually in the Methodology.

